Hyperbolic Image Embeddings

Computer vision tasks such as image classification, image retrieval and few-shot learning are currently dominated by Euclidean and spherical embeddings, so that the final decisions about class belongings or the degree of similarity are made using linear hyperplanes, Euclidean distances, or spherical geodesic distances (cosine similarity). In this work, we demonstrate that in many practical scenarios hyperbolic embeddings provide a better alternative.

==> tables/deltas.tex <==
\begin{table*}[htb!]
\caption{The relative delta $\sfrac{2\delta (X)}{\mathrm{diam}(X)}$ and curvature parameter values calculated for different datasets. For image datasets we measured the Euclidean distance between VGG16 features. $S_2$ and $S_2, z>0$ denote the two--dimensional unit sphere and upper hemisphere correspondingly (1700 points were sampled from each one). 
}
\label{tab:deltas}
\begin{center}
  \begin{tabular}{ccccccc}
    \toprule
   & {Tree} & {Omniglot} & {CUB} & {\textit{mini}ImageNet} & {$S_2$} & {$S_2,z > 0$}\\
    \midrule
   $\sfrac{2\delta (X)}{\mathrm{diam}(X)}$ & $0$ & $0.31$ & $0.23$ & $0.14$ & $0.99$ & $0.94$\\
    $c$ & - & $0.036$ & $0.005$ & $0.007$ & - & - \\ 
    \bottomrule
  \end{tabular}
\end{center}
\vspace{-5mm}
\end{table*}

==> tables/hyperparams_mini_1shot.tex <==
\begin{table}[]
\label{tab:hyp_1s_mini}
\begin{center}
\begin{tabular}{@{}lll@{}}
\toprule
          & \multicolumn{2}{c}{\textbf{Model}}                                          \\ \midrule
\textbf{} & \multicolumn{1}{c}{\textbf{4-Conv}} & \multicolumn{1}{c}{\textbf{ResNet18}} \\ \midrule
c         & 0.01                                & 0.001                                 \\ \midrule
lr        & 5e-3                                & 5e-3                                  \\ \midrule
gamma     & 0.5                                 & 0.5                                   \\ \midrule
step      & 80                                  & 80                                    \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/min_cub.tex <==
\begin{table*}[htb!]
% \caption{Experimental results on two datasets: \textit{Mini}ImageNet and CUB averaged over $10,000$ test episodes and are reported with $95\%$ confidence intervals.}
\caption{Experimental results on two datasets: \textit{Mini}ImageNet and CUB averaged over $10,000$ test episodes and are reported with $95\%$ confidence intervals. As the baseline model, we consider ProtoNet with the parameters described in Appendix ~\ref{app:details}. 
% The hyperbolic model is the generalization of the baseline model made by adding the mapping to Poincar\'e ball and substituting Euclidean mean operation to hyperbolic averaging. The obtained accuracy values indicate better performance of the hyperbolic model. 
% We may conclude that in these experiments transferring data into hyperbolic space and replacing the corresponding operations lead to higher accuracy values. 
We report the experimental results with different values of parameter $c$: the first is fixed for both datasets and equals $0.05$, and the remaining values were estimated using Gromov hyperbolicity (Table \ref{tab:deltas}).}
\label{tab:min_cub}
\begin{center}
  \begin{tabular}{llccc}
    \toprule
  {Dataset} &  {Model} & {$c$} & {1-shot 5-way} & {5-shot 5-way} \\
    \midrule
    \multirow{5}{*}{\textit{Mini}ImageNet} & MatchNet ~\cite{vinyals2016matching} &-& $43.56 \pm 0.84$ &$55.31 \pm0.73$\\
    & ProtoNet &-&$48.29 \pm 0.19$& $66.11 \pm 0.16$\\
    & RelationNet ~\cite{sung2018learning}  &-& $50.44 \pm 0.82$ & $65.32 \pm 0.70$ \\
    & Hyperbolic ProtoNet &$0.05$& $\mathbf{51.57 \pm 0.2}$ & $66.27 \pm 0.17$\\
    & Hyperbolic ProtoNet &$0.007$& $47.97 \pm 0.19$ & $\mathbf{68.92 \pm 0.16}$\\
    \midrule
    \multirow{3}{*}{CUB} & ProtoNet & - &$54.58 \pm 0.24$& $68.04 \pm 0.19$\\
    & Hyperbolic ProtoNet &$0.05$& $\mathbf{60.52 \pm 0.25}$ & $72.22 \pm 0.19$\\
    & Hyperbolic ProtoNet & $0.005$ & $58.03 \pm 0.24$ & $\mathbf{75.80 \pm 0.17}$\\
    \bottomrule
  \end{tabular}
\end{center}
\vspace{-5mm}
\end{table*}

% As the baseline model, we consider ProtoNet with the parameters described in Subsections \ref{subsec:min} and \ref{subsec:cub}. The hyperbolic model is the generalization of the baseline model made by adding the mapping to Poincar\'e ball and substituting Euclidean mean operation to hyperbolic averaging. The obtained accuracy values indicate better performance of the hyperbolic model. We may conclude that in these experiments transferring data into hyperbolic space and replacing the corresponding operations lead to higher accuracy values


==> tables/omni_siamese.tex <==
\begin{table}[htb!]
\caption{Comparison of the Euclidean and hyperbolic siamese networks in the $1$-shot $20$-way setting on the Omniglot dataset. Hyperbolic architectures use $\mathrm{Concat}$ based \eqref{eq:concat} similarity, and hyperbolic distance similarity correspondingly. Note that hyperbolic architectures outperform the Euclidean variant with significant margin. $c=1$ was used for this experiment.}
\label{tab:omni_siamese}
\begin{center}
  \begin{tabular}{rccc}
    \toprule
  {dim} &  {$128$} & {$256$} & {$512$} \\
    \midrule
    
  Euclidean similarity & $90.08$ & $91.03$ & $91.32$\\
  Hyperbolic $\mathrm{Concat}$  & $93.63$ & $94.23$ & $\mathbf{94.62}$\\ 
  Hyperbolic distance & $\mathbf{95.54}$ & $\mathbf{95.00}$ & $19.25$\\
    \bottomrule
  \end{tabular}
\end{center}
\end{table}

==> tables/reid_tr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[htb!]
\begin{tabular}{clllllllll}
\multicolumn{1}{l}{} &                                 & \multicolumn{4}{c}{market-1501}                                                                     & \multicolumn{4}{c}{duke}                                                                            \\
\multicolumn{1}{l}{} &                                 & \multicolumn{2}{c}{bs}                           & \multicolumn{2}{c}{hyp}                          & \multicolumn{2}{c}{bs}                           & \multicolumn{2}{c}{hyp}                          \\
dim                  & \multicolumn{1}{c}{lr schedule} & \multicolumn{1}{c}{r1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{r1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{r1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{r1} & \multicolumn{1}{c}{mAP} \\
\multirow{2}{*}{32}  & sch\#1                          & {\ul 71.4}             & {\ul 49.7}              & 69.8                   & 45.9                    & 56.1                   & 35.6                    & 56.5                   & 34.9                    \\
                     & sch\#2                          & 68.0                   & 43.4                    & \textbf{75.9}          & \textbf{51.9}           & {\ul 57.2}             & {\ul 35.7}              & \textbf{62.2}          & \textbf{39.1}           \\
\multirow{2}{*}{64}  & sch\#1                          & 80.3                   & 60.3                    & {\ul 83.1}             & {\ul 60.1}              & 69.9                   & 48.5                    & \textbf{70.8}          & \textbf{48.6}           \\
                     & sch\#2                          & 80.5                   & 57.8                    & \textbf{84.4}          & \textbf{62.7}           & 68.3                   & 45.5                    & {\ul 70.7}             & {\ul 48.6}              \\
\multirow{2}{*}{128} & sch\#1                          & 86.0                   & 67.3                    & \textbf{87.8}          & \textbf{68.4}           & {\ul 74.1}             & {\ul 53.3}              & \textbf{76.5}          & \textbf{55.4}           \\
                     & sch\#2                          & {\ul 86.5}             & {\ul 68.5}              & 86.4                   & 66.2                    & 71.5                   & 51.5                    & 74.0                   & 52.2                   

\end{tabular}
\end{table}
